A Longitudinal Analysis of a Social Network of Intellectual History

The history of intellectuals consists of a complicated web of influences and interconnections of philosophers, scientists, writers, their work, and ideas. How did these influences evolve over time? Who were the most influential scholars in a period? To answer these questions, we mined a network of influence of over 12,500 intellectuals, extracted from the Linked Open Data provider YAGO. We enriched this network with a longitudinal perspective, and analysed time-sliced projections of the complete network differentiating between within-era, inter-era, and accumulated-era networks. We thus identified various patterns of intellectuals and eras, and studied their development in time. We show which scholars were most influential in different eras, and who took prominent knowledge broker roles. One essential finding is that the highest impact of an era's scholar was on their contemporaries, as well as the inter-era influence of each period was strongest to its consecutive one. Further, we see quantitative evidence that there was no re-discovery of Antiquity during the Renaissance, but a continuous reception since the Middle Ages.

==> CommunityEvolution.tex <==

In order to get insights on whether intellectuals form communities based on their influence relationships.


%%=====================================
\subsection{Detecting Communities}

In a social network, a community can be considered as a set of entities that are closer to each other, compared to the rest of the entities in the network. 
We refer to Fortunato \cite{Fortunato:2010} as an extensive survey of existing approaches for community detection.
In particular, community detection in directed networks is more challenging task as compared to the undirected case. We refer to \cite{Malliaros:2013} for a survey on community detection in directed networks.

For our study we used the InfoMap two-level algorithm as implemented in the map equation framework \cite{Bohlin:2014}.
The core of the algorithm follows closely the Louvain method \cite{Blondel:2008}, where neighboring nodes are joined into modules, which subsequently are joined into supermodules and so on. 

First, we applied community detection on accumulative influence networks. At each era, the accumulative influence network consists of all influence links among actors who lived in that era or in any previous era (see Section \ref{sec:accumulative}).

Table \ref{tab:comms} shows for each era, the number of all detected communities ($C$), number of large communities ($LC$) (whose size is $\geq 10$), and the top three largest communities ($LC_1,LC_2,LC_3)$, with their number of nodes and edges.
We clearly observe how the number of communities increases over time, which is basically due to the increase in number of actors.
% that increasing the 
\begin{table}[H]
\centering
\caption{Detected Communities, $C$: No. of all communities, $LC$: no. of large communities (size$\geq 10$), $LC_i$: $i^{th}$ largest community}
\label{tab:comms}
\begin{tabular}{l | r | r | rr | rr | rr}
\multirow{2}{*}{Era} & \multirow{2}{*}{$C$} &
\multirow{2}{*}{$LC$} & 
\multicolumn{2}{c|}{$LC_1$} & 
\multicolumn{2}{c|}{$LC_2$} & 
\multicolumn{2}{c}{$LC_3$} \\
\cline{4-9}
 	  &     &      & N & E & N & E & N & E \\
\hline
Antiquity    &    33 &   9 & 24 & 47 & 13 & 13 & 13 & 12 \\
MiddleAges   &    82 &  19 & 27 & 53 & 21 & 31 & 17 & 26 \\
EarlyModern  &   205 &  37 & 34 & 47 & 33 & 58 & 29 & 52 \\
Sattelzeit   &   369 &  64 & 53 & 81 & 31 & 47 & 30 & 55 \\
ModernAge    &   742 & 135 & 60 & 108& 53 & 91 & 49 & 87 \\
Contemporary & 1,782 & 390 & 98 & 199& 97 &184 & 82 & 158 \\
\hline
\end{tabular}
\end{table}

Table \ref{tab:comms_members} gives an overview of the number of members of detected communities.

\begin{table}[H]
\centering
\caption{Number of community members}
\label{tab:comms_members}
\begin{tabular}{l | r  r | r r r r r}
Era         & mean & std & min & 25\% & 50\% & 75\% & max \\
\hline
Antiquity    & 6.70 & 4.84 & 2 & 3 & 5 & 10& 24 \\
MiddleAges   & 6.73 & 5.11 & 2 & 3 & 5 & 9 & 27 \\
EarlyModern  & 5.98 & 5.57 & 2 & 2 & 4 & 7 & 34 \\
Sattelzeit   & 5.80 & 5.84 & 2 & 2 & 3 & 7 & 53 \\
ModernAge    & 6.33 & 7.04 & 1 & 2 & 4 & 8 & 60  \\
Contemporary & 7.02 & 8.34 & 1 & 2 & 4 & 9 & 98 \\
\hline
\end{tabular}
\end{table}

\begin{figure}[H]
    \centering
    \includegraphics[width=.8\linewidth]{Longitudinal_Influence_Network/images/comms_size.pdf}
    \caption{Distribution of community size for each era}
    \label{fig:boxplot}
\end{figure}

Since we are looking at accumulative influence networks, a community at a given era, would include actors from that era and eventually from previous eras, getting more diverse in regards to their longitudinal composition.
The natural question here is how diverse those communities are. 
To answer this question, we first need to define a measure of diversity, where we opt to use the normalized entropy (aka, Shannon-Wiener diversity index \cite{Spellerberg:2003}).
The entropy is calculated as follows:
% $$ H' = -\sum_i p_i \log_2 {p_i}  $$
$$ H' = \frac{ -\sum_i p_i \log_2 {p_i} }{\log_2(6)} $$
where $p_i$ is the proportion of actors belonging to the i$^{th}$ era. 
As we have 6 eras, we need to normalize the entropy by dividing it by $\log_2 6$, 
% $$ H = \frac{H'}{ \log_2(6) } $$.
Thus, the normalized entropy ranges between 0 and 1. It takes its minimum value (0) when all actors belong to the same era, and it takes maximum possible value (1), when the members belong to all the 6 eras with equal numbers.



\begin{table}[H]
\centering
\caption{Diversity of detected communities}
\label{tab:comms_diversity}
\begin{tabular}{l | r r r r }
Era &   mean & std & 75\% & max \\
\hline
Antiquity    & 0  \\
MiddleAges   & 0.18 & 0.34 & 0.17 & 1.00 \\
EarlyModern  & 0.16 & 0.26 & 0.34 & 0.98 \\
Sattelzeit   & 0.16 & 0.23 & 0.41 & 0.89 \\
ModernAge    & 0.17 & 0.22 & 0.39 & 0.83 \\
Contemporary & 0.18 & 0.21 & 0.36 & 0.95 \\
\hline
\end{tabular}
\end{table}

\subsubsection{Discussion}

These communities show clear thematic distinctions. 

The biggest three communities in Antiquity are Classical Philosophers around Aristotle, Plato and Socrates, a cluster of Greek and Roman poets (Virgil, Ovid), and a community mirroring the political ties between the Indian Gupta and Mauryan dynasties and the Seleukid empire. 

The Classical Philosophers community survived into the Middle Ages as the biggest cluster, followed by a community of Persian Poets of Sufi Mystics and Sunni poets dating from 9th to the 13th century (Rumi), and two communities of equal size of Islam theologians (Ahmad Ibn Hanbal) and Christian theologians (Thomas Aquinus). 

In the Early Modern period, the biggest community is formed by Enlightenment scholars of political theory (Locke, Hobbes, Machiavelli), followed by the cluster of Classical Philosophers of Antiquity, and the Sufi Poets community. The fourth biggest cluster is merged from the Roman Poets with contemporary early Modern Poets of the Renaissance (Ludovico Ariosto), representing their interest in the Classical antiquity. The 9. biggest cluster is consisting mainly of Natural Philosophers and Mathematicians, and a surprising high concentration of Polymaths of that time (Leibniz, Ramon Llull, Roger Joseph Boscovich).

The biggest community of the Transitioning period consists of Christian Theologians and Mystics, again headed by Thomas Aquinus. The second biggest group consists of Theologians and Natural Philosophers, Mathematicians, and Astronomers around Baruch Spinoza, Descartes, and Leibniz. The Classical Philosophers constitute the third biggest cluster here, too.

In Modern age, a new group of Political Philosophers and Political Economists constitute the biggest community, merging from the Early Modern period. A cluster of Socialist thinkers are formed around Marx and Hegel in the second biggest group, followed again by Christian Theologians of Aquinus. Here, the fourth biggest communities is formed by Mathematicians and Logicians around Ludwig Wittgenstein and Bertrand Russel.

A community of Stand up Comedians and Actors form the biggest cluster in Contemporary time (Richard Pryor), followed by on the second place, Philosophers on Religion and Nation (Hegel, Kant, Kierkegaard, Goethe) and the science community of Mathematicians and Logicians around Wittgenstein and Russel, supplemented by Science Philosophers such as Karl Popper.

The communities detected revolve around the main influence of each scholar, and comprise of reasonable thematic groups. We could analyze this further by using each community as a stepping stone of \colorbox{pink}{further communal analysis}, which would allow us to \colorbox{pink}{differentiate between smaller sub-groups and sub-movements} within the scholarly communities. \colorbox{pink}{Maybe of the Science Cluster in Contemporary?}

\emph{Can we differentiate schools or fields? As in the contemporary science cluster: Do mathematicians form their own cluster, or are they intertwined with the science philosophers? Does this represent a non-differentiation between the fields? Are these scholars active as polygraphs ("Universalgelehrte"), or something close to it (more than 1-2 research fields)? Are there differences to previous eras science cluster?}


%%=====================================
\subsection{Tracking the Evolution of Communities}

% After detecting communities at each era, we would like to explore how those communities evolved over time.
In order to track the evolution of communities, we follow the approach of Greene et al. \cite{Greene:2010}.
Their model for dynamic community analysis is focused around the life cycle of communities, and the key events that characterise the evolution of dynamic communities, such as birth (emergence), death (dissolution), splitting, and merging.
The objective is to identify a set of \emph{dynamic communities} that are present in the network across one or more time steps.
Communities identified at individual time steps are referred to as \emph{step communities}: they represent specific observations of dynamic communities at a given point in time.
Each dynamic community $D_i$ can be represented by a time-line of its constituent step communities, ordered by time, with at most one step community for each step $t$.
The most recent observation in a timeline is referred to as
the \emph{front} of the dynamic community.

The fundamental events that can be used to characterise the evolution of dynamic communities can be formulated in terms of a set of rules covering step and dynamic communities \cite{Greene:2010} (see Figure \ref{}):

\begin{itemize}
\item Birth: The emergence of a step community observed at time $t$ for which there is no corresponding dynamic community.
\item Death: The dissolution of a dynamic community $D_i$ occurs when it has not been observed (i.e. there has been no corresponding step community) for at least d consecutive time steps. $D_i$ is subsequently removed from the set D.
\item Merge: A merge occurs if two distinct dynamic communities $(D_i, D_j )$ observed at time $t-1$ match to a single step community $C_{ta}$ at time $t$. The pair subsequently share a common timeline starting from $C_{ta}$.
\item Split: It may occur that a single dynamic community $D_i$ present at time t - 1 is matched to two distinct step communities $(C_{ta} , C_{tb} )$ at time $t$. A branching occurs with the creation of an additional dynamic community $D_j$ that shares the timeline of $D_i$ up to time $t - 1$, but has a distinct timeline from time $t$ onwards.
\end{itemize}

There are also trivial one-to-one matching or \emph{continuation} events where a dynamic community observed at time $t$ also has an observation at time $t + 1$. 

\begin{figure}[H]
\centering
\includegraphics[width=0.6\linewidth]{images/dynamic_communities.pdf}
\caption{Examples of evolution events according to \cite{Greene:2010}, from top down: continuation, birth, death, merge, and split.}
\label{fig:evolution_events}
\end{figure}


The strategy of tracking communities across time steps
is a heuristic threshold-based method, which allows for many- to-many mappings between communities across different time steps. 
The strategy proceeds as follows. 
Given the first step grouping $\mathbb{C}_1$ (communities of the first time step) a distinct dynamic community is created for each step community. 
Then, with the next grouping $\mathbb{C}_2$, an attempt is made to match these step communities with 
the fronts $\{F_1, \cdots, F_{k'}\}$ (i.e. the step communities from $\mathbb{C}_1$).
All pairs $(C_{2a}, F_i)$ are compared, and the dynamic community timelines and fronts are updated based on the event rules described previously. The process continues until all step groupings have been processed.

To perform the actual matching between $C_t$ and the fronts $\{F_1, \cdots , F_{k'} \}$, the widely-adopted Jaccard coefficient for binary sets is used. 
Given a step community $C_{ta}$ and a front $F_i$, the similarity between the pair is calculated as:

$$ sim(C_{ta}, F_i) = \frac{| C_{ta} \cap F_i |}{ | C_{ta} \cup F_i |} $$
If the similarity exceeds a matching threshold $\theta \in [0, 1]$, the pair are matched and $C_{ta}$ is added to the timeline for the dynamic community $D_i$.

The output of the matching process will naturally reveal series of community evolution events. A step community matching to a single dynamic community indicates a ``continuation", while the case where it matches multiple dynamic communities results in a merge event. If no suitable match is found for a step community above the threshold $\theta$, a new dynamic community is created for it.

We apply this tracking method on the detected communities over the six eras as time steps.

%%%=========================================

\subsection{Threshold Effect}

The results of the evolution tracking process are highly affected by the threshold parameter $\theta$. 
For example, when $\theta$ is set to 0, the pair of communities being compared will be considered a match if they share at least one member, whereas when $\theta$ is set to 0.5, they need to share at least half of their members in order to be considered a match.

In order to get insight on how the threshold parameter $\theta$ affects the results of the evolution tracking process, we repeated the tracking process with different values of $\theta$ ranging from 0 to 0.95, with increase of 0.05, and we recorded the following metrics: 
(1) number of dynamic communities,
(2) number of `continued' dynamic communities,
(3) number of `merged' dynamic communities, 
(4) number of members per community (mean, median, 75\% quantile, max), and 
(5) diversity per community (mean, median, 75\% quantile, max).

Figure \ref{fig:tracking_flat} shows the number of dynamic communities, all, continued, and merged.

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{Longitudinal_Influence_Network/images/tracking_flat.pdf}
\caption{Number of dynamic communities w.r.t the threshold $\theta$}
\label{fig:tracking_flat}
\end{figure}


\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{Longitudinal_Influence_Network/images/tracking_memdiv.pdf}
\caption{Caption}
\label{fig:tracking_memdiv}
\end{figure}


We also observed the patterns of communities per eras.



\begin{table}[]
\centering
\caption{Caption}
\label{tab:my_label}    
\begin{tabular}{c c c c c c | r r}
\rotatebox[origin=l]{90}{Antiquity} &
\rotatebox[origin=l]{90}{MiddleAges} &
\rotatebox[origin=l]{90}{EarlyModern} &
\rotatebox[origin=l]{90}{Sattelzeit} &
\rotatebox[origin=l]{90}{ModernAge} &
\rotatebox[origin=l]{90}{Contemporary} &
 count & avg size
\\ \hline 
% \X &    &    &    &    &     & 2 & 11 \\
%  \X & \X &    &    &    &     & 2 & 20 \\
%  \X & \X & \X & \X &    &     & 1 & 11 \\
%  \X & \X & \X & \X & \X &     & 1 & 38 \\
 \X & \X & \X & \X & \X & \X  & 3 & 15 \\
\hline 
    % & \X & \X &    &    &     & 2 & 23.5 \\
    % & \X & \X & \X &    &     & 2 & 15 \\
    & \X & \X & \X & \X & \X  & 3 & 21 \\
    % & \X & \X &    & \X & \X  & 1 & 41 \\
    % & \X &    & \X & \X & \X  & 1 & 21 \\
    % & \X &    &    & \X & \X  & 1 & 40 \\
    % & \X &    &    &    & \X  & 2 & 19 \\
\hline     
    &    & \X &    &    &     & 7 & 15.57 \\
    % &    & \X & \X &    &     & 2 & 23 \\
    % &    & \X & \X & \X &     & 2 & 19.5 \\
    &    & \X & \X & \X & \X  & 12 & 23 \\
    % &    & \X & \X &    & \X  & 1 & 23 \\
\hline     
    &    &    & \X &    &     & 23 & 15.78\\
    &    &    & \X & \X &     & 4  & 13.5 \\
    &    &    & \X & \X & \X  & 7  & 33 \\
    % &    &    & \X &    & \X  & 2  & 22.5 \\
\hline     
    &    &    &    & \X &     & 66 & 17.94 \\
    &    &    &    & \X & \X  & 35 & 22.17 \\
\hline     
    &    &    &    &    & \X  & 325 & 17.81 \\
    \end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Longitudinal_Influence_Network/images/dycomms2.pdf}
    \caption{Dynamic communities with merge events ($\theta=0.35$)}
    \label{fig:merged_dycoms}
\end{figure}

% \begin{table}[]
% \centering
% \caption{Caption}
% \label{tab:my_label}    
% \begin{tabular}{c c c c c c | r}
% \rotatebox[origin=l]{90}{Antiquity} &
% \rotatebox[origin=l]{90}{MiddleAges} &
% \rotatebox[origin=l]{90}{EarlyModern} &
% \rotatebox[origin=l]{90}{Sattelzeit} &
% \rotatebox[origin=l]{90}{ModernAge} &
% \rotatebox[origin=l]{90}{Contemporary} &
%  \#
% \\ \hline 
%  \X &    &    &    &    &     & 4 \\
%  \X & \X &    &    &    &     & 6 \\
%  \X & \X & \X &    &    &     & 1 \\
%  \X & \X & \X & \X &    &     & 1 \\
%  \X & \X & \X & \X & \X &     & 2 \\
%  \X & \X & \X & \X & \X & \X  & 16 \\
%  \X & \X & \X & \X &    & \X  & 1 \\
%  \X & \X & \X &    &    & \X  & 1 \\
%  \X & \X &    & \X & \X &     & 1 \\
% \hline 
%     & \X &    &    &    &     & 5 \\
%     & \X & \X &    &    &     & 6 \\
%     & \X & \X & \X &    &     & 6 \\
%     & \X & \X & \X & \X &     & 5 \\
%     & \X & \X & \X & \X & \X  & 26 \\
%     & \X & \X &    & \X & \X  & 1 \\
%     & \X &    & \X &    & \X  & 1 \\
%     & \X &    &    & \X & \X  & 1 \\
%     & \X &    &    &    & \X  & 2 \\
% \hline     
%     &    & \X &    &    &     & 19 \\
%     &    & \X & \X &    &     & 12 \\
%     &    & \X & \X & \X &     & 5 \\
%     &    & \X & \X & \X & \X  & 97 \\
%     &    & \X & \X &    & \X  & 3 \\
%     &    & \X &    & \X &     & 2 \\
%     &    & \X &    & \X & \X  & 1 \\
% \hline     
%     &    &    & \X &    &     & 53 \\
%     &    &    & \X & \X &     & 17 \\
%     &    &    & \X & \X & \X  & 119 \\
%     &    &    & \X &    & \X  & 4 \\
% \hline     
%     &    &    &    & \X &     & 158 \\
%     &    &    &    & \X & \X  & 293 \\
% \hline     
%     &    &    &    &    & \X  & 1222 \\
%     \end{tabular}
% \end{table}



==> Diffusion.tex <==

In order to get insight on how the influence spread  throughout the network, and how this spread change over time, we study the diffusion of influence throughout the network, similarly to \cite{Ghawi:2019c}.

We refer to the influence path formed as actors influenced by an original actor, influence other actors, as a \emph{cascade} and the original actor as the \emph{root} actor.
For each actor, we construct his influence cascade, by considering out-going edges starting from that actor.
However, in order to avoid exhaustive search (due to cyclicity), we construct actor's cascade as a directed acyclic graph (DAG), i.e., in case of reciprocal edges between a pair of nodes, we arbitrarily choose one of the reciprocal edges. Thus, the result we obtain is a directed acyclic graph (DAG), which we call henceforth a cascade.

In order to characterize the influence cascades, we employ the following features as used in \cite{Mathew:2018,Vosoughi:2018}:
\begin{itemize}
\item Size: the number of nodes in the DAG which are reachable from the root actor, i.e., the total number of unique actors involved in the cascade.
\item Depth: the length of the longest path from the root node of the cascade.
\item Average depth: the average path length of all nodes reachable from the root actor. 
\item Breadth: the maximum number of nodes present at any particular depth in the cascade.
\end{itemize}

For all actors, we extracted their cascade DAGs, and computed the properties of cascades: size, depth, average depth and breadth. 
Clearly, there are some nodes that do not have cascades, since they do not have successors, i.e., they are not influencers (about 44\% of all nodes). 
Therefore, the cascades we obtained are 6,970 corresponding to influencer actors, who have successors.

Figure \ref{tab:top5diff} shows for each era the top 5 scholars based on the four features of cascades.
We observe that top cascades by size and by breadth correspond to Antiquity intellectuals, whereas, top cascades by depth correspond to intellectuals of the Middle Ages (Islam theologians).


\begin{figure*}[]
\centering
\caption{Analysis of Influence Diffusion Cascades of Scholars. Table shows the top 5 scholars of each era.}
\label{tab:top5diff}
\small
\begin{tabular}{ l | l r | l r | l r| l r}
\hline
\rowcolor{Gray}
Era & \multicolumn{2}{c}{Size} & 
      \multicolumn{2}{c}{Depth}   & 
      \multicolumn{2}{c}{Avg. Depth} &
      \multicolumn{2}{c}{Breadth} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Antiquity}} 
& \textbf{Thales}              & \textbf{5725} & Moses  & 17 &
Moses	            & 9.4  & \textbf{Aesop}  & \textbf{2167} \\
& \textbf{Anaximander}         & \textbf{5724} & Aaron  & 17 & 
Aaron	            & 9.4  & \textbf{Philo the Dialecticia}n  & \textbf{2163} \\
& \textbf{Hesiod}              & \textbf{5723} & John the Evangelist     & 15   &
John the Evangelist & 8.0  & \textbf{Pasicles of Thebes}      & \textbf{2163} \\
& \textbf{Pherecydes of Syros} & \textbf{5722} & Clement of Alexandria   & 15   &
Speusippus          & 7.8  & \textbf{Diodorus Cronus}	     & \textbf{2163} \\
& \textbf{Pythagoras}          & \textbf{5721} & Athanasius of Alexandria & 15 &
Pasicles of Thebes  & 7.4 & \textbf{Thrasymachus of Corinth} & \textbf{2163} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{MiddleAges}} 
& Ja'far al-Sadiq    & 5478 & \textbf{Abū \d Hanīfa}	       & \textbf{20} 
& \textbf{Abū \d Hanīfa}   & \textbf{12.1} & Al-Ghazali	       & 2125 \\
& Harbi al-Himyari   & 5434 & \textbf{Abu Suhail an-Nafi}   & \textbf{20} 
& \textbf{Abu Suhail an-Nafi} & \textbf{12.1} & Al-Juwayni   & 2125 \\
& Jābir ibn Hayyān   & 5433 & \textbf{Hisham ibn Urwah}     & \textbf{20} 
& \textbf{Hisham ibn Urwah}     & \textbf{12.1} & Abu Talib al-Makki    & 2125 \\
& Muhammad           & 5402 & \textbf{Malik ibn Anas}        & \textbf{19} 
& \textbf{Al-Juzajani} & \textbf{11.2} &  Harith al-Muhasibi & 2125 \\
& Al-Kindi           & 5401 & \textbf{Al-Shaybani}  & \textbf{19} 
& \textbf{Ibn Jurayj} & \textbf{11.2} & Al-Balkhi & 2104 \\

\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{EarlyModern}} 
& Nicholas of Cusa & 5203 & William Derham & 17 
& Jan van Scorel & 9.2 & Samuel Richardson & 2126 \\
& Michel de Montaigne & 5180 & John Ray & 17 
& William Derham & 8.5 & Denis Diderot & 2118 \\
& Francisco Suárez & 5175 & Giulio Cesare Croce & 17 
& John Ray & 8.5  & G-F. Rouelle & 2118 \\
& Gemistus Pletho & 5172 & N. Boileau-Despréaux & 16 
& Giulio Cesare Croce & 8.5 & Pierre Bayle & 2114 \\
& Basilios Bessarion & 5170 & Thomas Gray & 15 
& M. van Heemskerck & 8.2 & John Selden & 1965 \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Transition}} 
& J. N. Tetens & 4699 & H. T. Buckle & 18 
& F. K. Forberg   & 9.9  & Oliver Goldsmith & 1960 \\
& J. H. Lambert  & 4699 & J-F. Millet & 18 
& J-F. Millet     & 9.3  & Goethe & 1895 \\
& Immanuel Kant            & 4698 & Monticelli & 17 
& H. T. Buckle & 9.1  & James Macpherson & 1866 \\
& Thomas Reid         & 4644 & F. K. Forberg & 17 
& Bettina von Arnim   & 8.9  & F. G. Klopstock & 1844 \\
& J. G. Hamann & 4641 & Costache Caragiale & 16 
& A. P. de Candolle & 8.6 & Friedrich Schiller & 1838 \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{ModernAge}} 
& Hippolyte Taine & 3675   & Anton Mauve     & 17 
& Alfred Binet    & 9.1    & Hippolyte Taine & 1357 \\
& African Spir    & 3536   & Edmund John     & 17 
& James Mark Baldwin & 9.1 & African Spir    & 1283 \\
& Jean-Marie Guyau & 3256  & Thomas Mann     & 17 
& Jacob L. Moreno  & 9.1   & Herbert Spencer & 1071 \\
& Paul Bourget     & 3253  & Georges Seurat  & 17 
& E. E. Cummings   & 9.0   & Nietzsche       & 1008 \\
& Paul Rée         & 3253  & Vasile Pogor    & 17 
& Hans Vaihinger   & 8.9   & Paul Bourget    & 1008 \\

\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Contemporary}} 
& R. E. Schultes    & 884 & Witold Gombrowicz & 15 
& Kenneth Patchen   & 8.0 & Jean Genet        & 214 \\
& Witold Gombrowicz & 857 & Kenneth Patchen   & 15 
& Witold Gombrowicz & 7.9 & Henry Miller      & 193 \\
& Kenneth Patchen   & 857 & Thomas Bernhard   & 14 
& Robert Duncan     & 7.2 & R. E. Schultes    & 155 \\
& Robert Duncan     & 856 & Allen Ginsberg    & 14 
& Allen Ginsberg    & 7.1 & J-T. Desanti      & 154 \\
& Thomas Bernhard   & 853 & Robert Duncan     & 14 
& Thomas Bernhard   & 6.9 & J. L. Austin      & 148 \\

\hline
\end{tabular}
\end{figure*}

However, in order to get insight on how the features of those cascades evolve over time, we compare them over the consecutive eras as shown in Figure \ref{fig:cascades_features}.  
For each of the four features, size, depth, avg. depth, and breadth, we plot the mean, median, 75\% quantile and max. of the feature over the eras.
At a glance, one can see that the size and breadth features exhibit similar behaviors; and the depth and avg. depth features exhibit similar behaviors as well.  
The mean size decreases smoothly over time until it almost vanishes at Contemporary period.
The maximum size also decreases but slower than the mean size. Surprisingly, the median size vanishes quickly, i.e., it drops from about 5,000 at Antiquity to about 0 at Middle Ages and stay so at subsequent eras. This means that at least half of actors at each era (except Antiquity) have nearly empty cascades. 

The depth feature (mean) also decreases smoothly from one era to another. The 75\% quantile of depth feature still constant (at 11) until Transition period, and drops afterwards. 
The maximum depth is rather constant (slight changes in the range [15,20]) over all eras, taking its highest value at Middle Ages.
The behavior of the avg. depth feature is similar to this of the depth. The breadth feature has a similar behavior to the size feature.

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{Longitudinal_Influence_Network/images/cascades_features.pdf}
\caption{Evolution of cascades features over time}
\label{fig:cascades_features}
\end{figure}

The correlation between the size and breadth features, and the correlation between the depth and avg. depth features can be seen in Figure \ref{fig:cascades_corr} that shows the correlation matrix of the four features.
Those values are almost the same over all eras.

\begin{figure}[H]
\centering
\includegraphics[width=.52\linewidth]{Longitudinal_Influence_Network/images/cascades_corr.pdf}
\caption{Correlation matrix of cascades features}
\label{fig:cascades_corr}
\end{figure}

%%===========================================
\subsubsection{Clustering}

To get more insight on how the cascades correlate over the different eras, Figure \ref{fig:cascades_scatter} shows scatter plots of pairs of those features \footnote{Such scatter plots have been also constructed in \cite{Ghawi:2019c}}.
One can clearly observe how the points corresponding to the same era are clustered together, with smaller values roughly correspond to recent eras, whereas larger values correspond to early eras.

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{Longitudinal_Influence_Network/images/cascades_scatter.pdf}
\caption{Correlation of cascades features over eras}
\label{fig:cascades_scatter}
\end{figure}

In \cite{Ghawi:2019c}, a clustering approach was used to categorize influence cascades based on their aforementioned features, where two major categories of small and large cascades were identified and characterized.
The emergence of the cluster of large cascades has been interpreted in \cite{Ghawi:2019c} to be due to temporal dimension, claiming that most of the intellectuals in this cluster belong to Antiquity and Middle Ages.

Here we have the opportunity to verify this hypothesis, as we have the assigned eras of actors.
We apply K-Mean clustering algorithm \cite{Lloyd:1982,MacQueen:1967}, using the four features of cascades, size, breadth, depth, and avg. depth.
We applied this algorithm twice, using $k = 2$ and $k=6$ as the number of desired clusters.
The objective of clustering into two clusters is to verify the


\begin{table}[H]
\centering
\caption{Caption}
\label{tab:my_label}
\begin{tabular}{l |  r r r | r r r |}
\hline
           & \multicolumn{3}{c|}{Small Cascades} 
           & \multicolumn{3}{c|}{Large Cascades}  \\
count      & \multicolumn{3}{c|}{5815} & \multicolumn{3}{c|}{1155}  \\
\hline
           &mean & [min, & max] & mean & [min, & max] \\
\hline           
Size       & 26.0 & 1     & 1254 & 3136 & 350 & 5725   \\  
Depth      &  2.3 & 1     & 12   & 12   &   8 &   20   \\
Avg. Depth &  1.6 & 1     & 8.1  & 5.6  & 3.4 & 12.1   \\
Breadth    &  9.1 & 1     & 389  & 987  & 94  & 2167   \\
\hline
\end{tabular}

\vspace{1em}
\begin{tabular}{l |  r r  | r r  |}
Antiquity    &    55 & (29\%)   &  137 & (71\%)    \\
MiddleAges   &   130 & (54\%)   &  112 & (46\%)    \\ 
EarlyModern  &   304 & (59\%)   &  212 & (41\%)    \\
Transition   &   474 & (61\%)   &  305 & (39\%)    \\
ModernAge    & 1,630 & (81\%)   &  376 & (19\%)   \\
Contemporary & 3,222 & (100\%)  &   13 &  (0\%)   \\
\end{tabular}

\end{table}


\begin{figure}
\centering
\includegraphics[width=\linewidth]{Longitudinal_Influence_Network/images/cascades_clustering.pdf}
\caption{Clustering of influence cascades, using 2 clusters, and 6 clusters}
\label{fig:cascades_clustering}
\end{figure}

%%===========================================
\subsubsection{Classification}




==> _Analysis.tex <==



\subsection{Exploratory Data Analysis}


Our data set comprises 22,485 directed influence links among 12,506 scholars embedded into 6 historical eras. Figure \ref{fig:nActors} shows each era's continuous density of scholars based on their lifespan.

With scholars embedded in their respective eras, the entire influence network can be time-sliced: we project it into several partial networks based on the source era (of the influencer) and target eras (of the influenced scholar). When the source and target eras are the same, we called the partial network a \emph{within-era} influence network. When the source and target eras are different, we called the partial network an \emph{inter-era} influence network. There are no reverse links from an later era to a previous one due to pre-processing.

After time-slicing the whole network, we received
six within-era networks corresponding to all the six eras, and 15 inter-era networks, corresponding to all chronologically ordered but not necessarily consecutive pairs of different eras.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/heatmap.pdf}
\caption{Number of influence links from preceding periods (rows) to target eras (columns)}
\label{fig:heatmap}
\end{figure}

Figure \ref{fig:heatmap} shows the number of influence links among all pairs of eras. 
% Rows represent source eras, and columns represent target eras, i.e., each cell displays the number of influence links incoming from (actors in) the row era, outgoing to (actors in) the columns era.
% One can easily observe that the greatest deal of links occur within the Contemporary era, followed by the links from Modern Age to Contemporary, and within Modern Age. This is obviously because those recent eras comprise the largest deal of scholars in our data set.
The vast majority of links occured within the Contemporary era, followed by links from Modern Age to Contemporary, and within Modern Age, which is clearly owed to the increased amount of scholars in these periods. 
Noteworthy is also the spike in the influences of Antiquity on the Early Modern Period, which represents their increased reception during the Renaissance. % also different periodizations for Renaissance available: 15/16th century vs 1350-1650 with various stages, e.g. ean-Marie Le Gall, Défense et Illustration de la Renaissance, (Paris, PUF, 2018) or https://bmcr.brynmawr.edu/2020/2020.03.54
The links of Antiquity to the Middle Ages reassert the shift in historical research that the Renaissance did not "re-discover" Antiquity, but was received before in the Middle Ages as well \cite[p. 3-4]{fejfer:2003}. 

An interesting observation is that in general the highest fraction of influence received by the scholars of each era come from its own era. This means that the internal impact of any era is in general higher than its external impact.
This fact can be observed in Figure \ref{fig:inflc_pc}, which shows the percentage of influence of eras on each other. 
As our earliest period, Antiquity received only influence links from itself, whereas the influence received in the Middle Ages are 82\% internal, and 18\% from Antiquity. Subsequently, the amount of the within-era influence shrinks throughout the consecutive periods, but still remains the biggest influence. 

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{images/inflc_pc.pdf}
\caption{Percentage of received influences in each era.}
\label{fig:inflc_pc}
\end{figure}


%%==================================================
% \subsection{Independent Influence Networks}
% \label{sec:independent}
\input{section/sub_independent}
%%%==================================================
\subsection{Accumulative Influence Networks}
\label{sec:accumulative}
\input{section/sub_accumulative}

==> data_1.tex <==

We are studying scholars included at
% Our main data source is 
YAGO (Yet Another Great Ontology) \cite{Suchanek:2007,yago:2015}, which is a huge semantic knowledge base, developed at the Max Planck Institute for Computer Science in Saarbr\"ucken. 
YAGO was among the first projects to extract semantic knowledge at a large scale from Wikipedia. Together with DBpedia \cite{dbpedia:2009}, it is one of the pioneering contributors of Linked Open Data (LOD).
Currently, YAGO contains more than 10 million entities and more than 120 million facts about these entities. The information in YAGO is extracted from Wikipedia\footnote{https://www.wikipedia.org/} (e.g., categories, redirects, infoboxes), WordNet \cite{Miller:1995} (e.g., synsets, hyponymy), and GeoNames\footnote{http://www.geonames.org/}. 
% The accuracy of YAGO was manually evaluated to be above 95\% on a sample of facts. 
To integrate it to the linked data cloud, YAGO has been linked to the DBpedia ontology\footnote{http://www.mpi-inf.mpg.de/departments/databases-and-information-systems/research/yago-naga/yago/linking/} and to the SUMO ontology\footnote{http://www.mpi-inf.mpg.de/~gdemelo/yagosumo/}.

% Linked open data are typically represented using RDF (Resource Description Framework), which is the W3C standard for representing information in the Semantic Web \cite{rdfprimer:2004}. RDF is based on a directed graph data model, where both nodes and edges are labelled. A RDF graph is a set of triples of the form $(s,p,o)$, which can be interpreted as edges labelled by $p$ (the predicate) from nodes labelled by $s$ (the subject) to nodes labelled by $o$ (the object). 
% SPARQL, which became a W3C recommendation in 2008, is the standard query language for RDF \cite{sparql:2008,sparql:2013}.

As argued by Ghawi et al. in \cite{Ghawi:2019}, LOD can be used as a source of information to extract social networks among entities, called \emph{direct extraction} pattern.
% This technique to extract social networks from LOD is called \emph{direct extraction} pattern, as described in \cite{Ghawi:2019}, 
A case study has been presented in \cite{Ghawi:2019b}, where this \emph{direct extraction} is used with \verb|yago:influences| predicate to extract \emph{ego-centric} networks of several intellectuals. 
Other extraction patterns, such as \emph{derivation}, are also described in \cite{Ghawi:2019,Ghawi:2019b}.

We are particularly interested in the \verb|yago:influences| predicate that relates intellectuals based on their influence relationship. The confidence score of this relation is 0.96, as calculated by YAGO.

To extract our target influence social network, we used a SPARQL query as shown in Figure \ref{fig:query}. 
The query has been executed over YAGO's SPARQL endpoint.\footnote{{https://linkeddata1.calcul.u-psud.fr/sparql}, as of July 2019.}
The result of the query is a list of 22,818 records, where each record has two elements labeled $u$ and $v$, which represent two actors (intellectuals) where $u$ influences $v$. These records represent the edges of our target social network of influence.
Overall, these links connect 12,705 actors which constitute the nodes of the network.

\begin{figure}[H]
\centering
\caption{SPARQL query used to extract the influence social network}
\label{fig:query}
\begin{lstlisting}
SELECT ?u ?v
WHERE {
  ?u yago:influences ?v.
}
\end{lstlisting}    
\end{figure}

The scholars included at YAGO are persons involved in .... {\color{pink}{what are the definition of scholars there?}}
{\color{green}{there is none! there is only this `influences' relation connecting entities, which even are not necessarily persons!}}
% "political thought and culture, philosophy, religion, literature and literary criticism, social and natural sciences, visual arts and aesthetic theory, communications, law, economic thought, psychology, anthropology, music and the history of the book" 
% \citep[Definition of Journal of Modern Intellectual History, p. 136]{subrahmanyam review}. 
YAGO records only the most important influences and influenced persons, so we have a reduced version of a complex web of inter-dependencies {\color{red}{oida!}}.

This influence network has been analyzed in detail in \cite{Ghawi:2019c}.

In order to incorporate a time dimension to our data and analysis, we also extracted the birth and death dates of the actors. We used the SPARQL query shown in Figure \ref{fig:query2}, where the predicates \verb|wasBornOnDate| and \verb|diedOnDate| are used to retrieve birth and death dates of the actors, respectively. Since an actor could be influenced or an influencer, their entity would appear in the subject or object positions of the triple pattern. Therefore, the query contains a combination of both patterns using a \verb|UNION| operator. Finally, since the data set may not have information about the birth date or the death date (or both) of some actors, the triple patterns to retrieve those dates are stated as optional.


\begin{figure}[H]
\centering
\caption{SPARQL query to extract birth and death dates}
\label{fig:query2}
\begin{lstlisting}
SELECT ?u ?birthDate ?deathDate
WHERE {
  { SELECT DISTINCT ?u WHERE {
      { ?u yago:influences ?v. } 
       UNION 
      { ?v yago:influences ?u. }
  } }
 OPTIONAL {?u yago:wasBornOnDate ?birthDate.}
 OPTIONAL {?u yago:diedOnDate    ?deathDate.}
}
\end{lstlisting}    
\end{figure}

The results of this query are as follows:

\begin{itemize}
\item 8,073 have both dates (119 of them had errors: death dates before birth dates, which had to be manually corrected).
\item 4,030 have birth date, but no death date (hence, death dates were deduced by adding 60 years to the birth date, up to the symbolic year of 2020).
\item 82 have death date, but no birth date (birth dates were deduced by subtracting 60 years from the death date).
\item 520 have neither dates.
\end{itemize}

For the remaining 520 actors with neither dates, we used a SPARQL query to get the equivalent entities in DBpedia dataset using \verb|owl:sameAs|. Then, using these entities, we were able to extract the birth and/or death dates from DBpedia for 196 actors. 
Finally, we had to verify the remaining 324 cases manually to get their dates.
During this verification, we had to remove 128 entities, as they do not actually correspond to intellectuals. Those removed entities were either 1) concepts, e.g., `German\_philosophy' and `Megarian\_school', 2) legendary characters, e.g., `Gilgamesh' and `Scheherazade', or 3) bands e.g., `Rancid' and `Tube'. 

% We also adjusted X instances, where sender and receiver were confussed.
% ( This point is discussed later)


To this end, we obtained a new data set of 12,577 actors with complete dates of birth and death.



